"It was 80% me, 20% AI": Seeking Authenticity in Co-Writing with Large Language Models

Given the rising proliferation and diversity of AI writing assistance tools, especially those powered by large language models (LLMs), both writers and readers may have concerns about the impact of these tools on the authenticity of writing work. We examine whether and how writers want to preserve their authentic voice when co-writing with AI tools and whether personalization of AI writing support could help achieve this goal. We conducted semi-structured interviews with 19 professional writers, during which they co-wrote with both personalized and non-personalized AI writing-support tools. We supplemented writers' perspectives with opinions from 30 avid readers about the written work co-produced with AI collected through an online survey. Our findings illuminate conceptions of authenticity in human-AI co-creation, which focus more on the process and experience of constructing creators' authentic selves. While writers reacted positively to personalized AI writing tools, they believed the form of personalization needs to target writers' growth and go beyond the phase of text production. Overall, readers' responses showed less concern about human-AI co-writing. Readers could not distinguish AI-assisted work, personalized or not, from writers' solo-written work and showed positive attitudes toward writers experimenting with new technology for creative writing.

==> archived/initial_submission.tex <==
\section{Introduction}

From text suggestion \cite{Mina_Lee_CoAuthor} and summarization \cite{AIwriting_auto_summary} to style transformation \cite{AIwriting_Tool_arbitrary_style_transfer}, metaphoric generation \cite{AIwriting_metaphorian}, and information synthesis \cite{news_summ_eval_2022}, burgeoning applications of artificial intelligence (AI) for text production are rapidly reshaping writing experiences and practices, especially with the recent prominent releases of large language models (LLMs). 
Consequently, vast transformations of the writer economy are likely underway.
Within such a climate, seeking and preserving \textit{\textbf{authenticity}}---as a cornerstone for all forms of creation---in writing artifacts co-created with AI may become an increasingly complicated yet critical matter for writers. 


Indeed, existing literature has pointed to the importance of understanding authenticity for several reasons:
From author-centered perspectives, authenticity determines the value of their work, and co-writing with AI can potentially pose threats to this core value~\cite{HAIC_authenticity_Social_Dynamics_Gero}.
Moreover, writing serves as the medium for writers to connect with their audiences, and authentic expression contributes to the soundness of such bonds~\cite{writer-reader_Candlin_Hyland_1999, writer-reader_sharing_words, writer-reader_writing_for_readers}.
A deeper understanding of authenticity also facilitates discussions around ownership of work \cite{HAIC_authenticity_AI_Ghostwriter_Effect} as well as their relevant practices, e.g., declaring authorship, regulating copyright, detecting plagiarism, and commissioning writers' work. 
% -- as human-AI co-creation becomes commonplace \tocite{}.
Recent work has begun to explore relevant constructs, such as ownership, authorship, and agency~\cite{mieczkowski2022ai, HAIC_authenticity_AI_Ghostwriter_Effect, HAIC_authenticity_choice_over_control, HAIC_tool_agency}, 
%such as agency AI writing assistance \tocite{} and perceived authorship of AI-generated text \tocite{}.
but more comprehensive views of authenticity in human-AI co-creation remain vague.
% Meanwhile, public discussions reveal growing concerns about the potential threats of AI assistance tools to creators' value and authenticity in their work \cite{news_Lee_2023}.
Though public discussions reveal growing concerns from writers~\cite{news_Lee_2023}, it remains unclear how they would like to preserve their authentic voices in writing.


Meanwhile, personalized AI applications---including the \textit{personalization of AI writing assistance}---are becoming more common and readily accessible~\cite{personalization_CIKM_workshop, personalization_NLG, personalization_social_media_misinfo, personalization_user_centric_TTT}. This is especially promising with LLMs, which can often be guided to generate a specific form or style of text through natural language based prompting techniques, also allowing people without much AI/ML expertise to experiment with personalizing or steering the type of text being generated. 
%With emergent features (e.g., fine-tuning, prompting, in-context learning) powered by large-language models (LLM), even users without much AI/ML expertise could easily custom-build their AI writing assistance. 
For instance, a user could try to personalize AI suggestions to simulate their own writing style by specifying the characteristics in the prompt or by providing just a few of their own writing samples (i.e. in-context learning~\cite{brown2020language}).
Nonetheless, is personalization sufficient to preserve writers' authentic voices in writing?
While some recent research might suggest personalized AI adds little to authors' perceived ownership of their co-created writing work with AI~\cite{HAIC_authenticity_AI_Ghostwriter_Effect}, the concerns about and potential of personalization in supporting authenticity remain largely under-explored.

% Vera's comments:
% Another research gap/motivation is to study personalization. I think we can highlight LLMs’ opportunities for easy personalization, possible benefits of personalization for authenticity, and post it as an open question, e.g. “ different from previous generation of AI or automated writing support tools, LLMs allow for easy adaptation (e.g. through fine-tuning, prompting including incontext learning). This opens up possibilities for writer to personalize the model and better inject their own styles in the generation. However, it remains an open question whether writers and readers perceive writing done with personalized laguage models to be more authentic [while a recent study found that personalization had little effect on related constructs such as perceived author ownership (https://arxiv.org/pdf/2303.03283.pdf [AI Ghostwriter Effect])---this paper is very relevant, but my understanding is they tested actually personalized v.s. placebo personalized, not exactly personalized v.s. non-personalized

%Given these various motivations, the present work takes 
In this work, we take a closer look at authenticity in writing from both writers' and readers' perspectives. 
We focus on what writers seek for authenticity as new practices of co-writing with AI emerge and whether personalization could support their goals.
% Furthermore, as personalized AI tools become readily available, we seek to understand the possible impact of personalization on writers' authentic voices in writing.
Specifically, we ask:
\begin{itemize}
    \item RQ1: How do writers and readers conceptualize authenticity in the context of human-AI co-writing?
    \item RQ2: Based on their conceptions of authenticity, do writers want to preserve their authentic voices in writing, and if so how?
    \item RQ3: Can personalized AI writing assistance support authenticity and help preserve writers' authentic voices (if desired) in writing, and if so how?
\end{itemize}
%\textbf{\textit{How do writers and readers conceptualize authenticity in the context of human-AI co-creation?}}
We examined these inquiries first through semi-structured interviews with 19 professional writers across various literature genres.
During the interviews, writer participants reflected on their conceptions of authenticity in writing \textit{and} co-writing with AI through situated experiences. 
Namely, they engaged in writing with both generic and personalized AI writing assistance powered by a state-of-the-art large language model (i.e., GPT-4).
We then complemented writers' perspectives with those from avid readers (N = 30), which allows us to gauge audiences' responses to writers co-writing with AI and their perception of the authenticity of such work.


%Findings of the current study provide new insights into this knowledge space.
Our findings provide new insights into how writers and readers perceive co-writing with AI writing support. 
To begin with, writer-centered conceptions of authenticity focus more heavily on the internal experiences of writers and extend beyond the constructs of authenticity from prior literature (i.e., authenticity as source, category, and value of creators' work)~\cite{Auth_Humanity_Guignon_2008, Auth_Humanity_Handler_1986, Auth_Humanity_Art_Newman_Bloom_2012}.
Furthermore, the use of AI in writing calls questions to the identity of content producer and the representativeness of the human writer, posing threats to authenticity in writing.
Meanwhile, the actual practices of co-writing with AI prompts writers to re-think the meaning of authenticity.
This suggests that the design of AI writing assistance tools can play a key role in (re-)shaping the concept of authentic writing.
Finally, in contrast to writers' concerns, readers express great interest in the new gradient of authentic writing where AI's contributions come into play.


Together, our work makes three key contributions:
(1) By contributing to the theoretical realm, we deepen the understanding of authenticity in the context of human-AI co-creation. We consolidated writer-centered definitions of authenticity, which include new aspects of authenticity that have not been emphasized in existing theories. %by highlighting both writers' and readers' points of view and extending theoretical constructs of authenticity in co-writing with AI.
(2) Our study offers several practical implications for the design of next-generation AI-powered co-writing tools, ranging from supporting writers' motivations, needs, addressing current pain points, to the formats and temporal considerations of AI writing assistance.
Beyond possible aids for productivity and creativity---as often discussed in prior literature, design implications revealed through our study place an additional requirement for preserving authenticity in writing.
(3) To gauge the impact of generative AI at societal scales, we discuss our theoretical and design implications alongside the increasingly prevalent practices of personalizing AI applications, re-examining whether individuals' authentic voices are amplified or lost as they convey messages through AI-powered tools to their broader audiences.



\section{Background \& Related Work}

\subsection{Roots of Authenticity in Human Creative Work}
Humanity and social science literature have long acknowledged authenticity as the core of human creative work \cite{Auth_Humanity_Guignon_2008, Auth_Humanity_AMA_Lehman_2019, Auth_Humanity_Art_Newman_Bloom_2012}.
Though there is a long-standing history of proposing theoretical frameworks for authenticity, researchers have not yet formed a consensus.
Still, they have often adopted three key themes to define and conceptualize authenticity: \textit{category}, \textit{source}, and \textit{value} \cite{Auth_Humanity_Guignon_2008, Auth_Humanity_Handler_1986, Auth_Humanity_AMA_Lehman_2019, Auth_Humanity_Creative_Persona, Auth_Humanity_Images_Charmé_1991, Auth_Humanity_Varga_Guignon_2023, Auth_Humanity_Art_Newman_Bloom_2012, Auth_Humanity_Lightness_Safran_2017, Auth_Humanity_Integral_Humanity_Anderson_1993, Auth_Humanity_Expressive_Authenticity_Lindholm_2013}.
First, the \textbf{\textit{Category}} theme concerns whether a piece of work matches one’s existing beliefs for its associated category. 
The scope of a category can vary, such as ranging from a particular style or school of work (e.g., Bauhaus-style architecture) to a certain era (e.g., a Renaissance painting).
Second, the idea of authentic \textbf{\textit{Source}} concerns whether one can trace a piece of work to a specific source (e.g., a person, a place, an event, or any type of origin).
This explains the importance of crediting authors and labeling the origins of work.
In particular, when work from certain individuals is truly one-of-a-kind---such as the highly recognizable work of Picasso, the audiences can easily identify them as the source of content.
In such cases, the concepts of \textit{category} and \textit{source} become more blended and interchangeable. 
\textit{\textbf{Value and alignment}} addresses the consistency between a creator’s internal states and their external expression.
Oftentimes in literature, scholars discuss whether creators could genuinely express themselves through text or, rather, speak in others' voices.

In our study, we explore whether writers' perceptions of authenticity in writing align with these constructs of authenticity for broader creative work and whether specific concerns apply to writing. Based on writer-centered definitions of authenticity, we further examine whether co-writing with AI is considered authentic and whether the emerging technologies change writers' view toward the essence of authenticity.

%\textit{RQ1a: How do writers define authenticity in writing?}

%\textit{RQ1b: Based on their definitions of authenticity, do writers consider co-writing with AI authentic writing?}

%\textit{RQ1c: Whether and how do writers' responses to RQ1a and RQ1b change after co-writing with AI?}


\subsection{The Impact of AI Use on Authenticity in Writing}

\subsubsection{Writers' increasing concerns regarding AI writing assistance}
The increasing popularity of using AI for creative tasks has motivated recent work to investigate the possible impact of AI on several aspects of creators' work (e.g., credit, authorship, ownership, control, and agency)~\cite{HAIC_authenticity_AI_Ghostwriter_Effect, HAIC_authenticity_Diffusing_Creator, HAIC_authenticity_Designing_Participatory_AI, HAIC_authenticity_choice_over_control}, many of which are closely related to authenticity.
Up to date, studies, workshops, panels, and numerous forms of discussion~\cite{news_Lee_2023} revealed mixed opinions from the public and the research communities toward these topics.
Here, we summarized a few emergent themes: %yet inconclusive themes:


\textbf{\textit{Writers remain hesitant to declare AI co-authorship publicly.}}
% [AI ghostwriter effect] 
%Writers don’t consider themselves as owners of AI-generated text, but they also refrain from publicly declaring AI authorship.
Recent work on perceived authorship of AI-generated text revealed an intricate \textit{AI Ghostwriter Effect}~\cite{HAIC_authenticity_AI_Ghostwriter_Effect}.
Through comparing personalized and pseudo-personalized AI tools, the findings suggest that though writers did not perceive complete ownership over AI-generated text, they were also reluctant to publicly declare AI co-authorship.
This reluctance could relate to writers' concerns about negative responses from their readers~\cite{HAIC_authenticity_Social_Dynamics_Gero}.
But more importantly, authorship should come hand in hand with the degree of contribution one makes to a piece of work~\cite{HAIC_authenticity_Diffusing_Creator}, although it remains unclear what constitutes \textit{contribution} from AI. 
% On the other hand, what makes meaningful human contributions when co-writing with AI may also remain an open question.
Moreover, it is generally challenging to specify which parts of the writing process make more meaningful contributions than others.


\textbf{\textit{Writers suspect AI would negatively impact their writing outcomes.}}
In several studies, writers expressed concerns that AI might distract them from their original ways of writing, causing lower quality of work~\cite{HAIC_authenticity_Designing_Participatory_AI}.
Besides, writers often raised the question of whether readers would be able to tell if they were using AI to write~\cite{HAIC_authenticity_Social_Dynamics_Gero}.
As shown in several studies, audiences could react negatively once they knew a piece of text was generated by AI~\cite{HAIC_authenticity_LLM_persuasion, HAIC_authenticity_Opinionated_LLM, HAIC_authenticity_Synthetic_Lies, AIwriting_self-presentation}.
It remains however unclear whether adverse reactions ensue regardless of the context in which AI is being used, or whether certain use cases of AI writing assistance are more acceptable.


\textbf{\textit{Writers worry that working with AI might deprive their control and joy during the writing process.}}
In general, writers hope to maintain control throughout their writing process~\cite{HAIC_authenticity_choice_over_control}.
Writers' sense of control not only shapes their perceptions of ownership of work but also whether  they are using AI as a tool or being influenced by AI~\cite{HAIC_tool_agency}.
As such, participants of a recent study expressed strong preferences for taking AI suggestions from multiple options instead of adopting a single, complete piece of AI-generated writing \cite{HAIC_authenticity_choice_over_control}.
From a job satisfaction perspective, writers also wondered whether working with AI would harm the degree to which they enjoy the process of writing \cite{HAIC_authenticity_Artificial_Colleague, HAIC_authenticity_Social_Dynamics_Gero}.


% [Social dynamics of AI support in writing] 
% Authenticity is a key value for writers. They are not only worried that (a) writing with AI would shift them away from their genuine voices but more about (b) whether their audiences would be able to identify such shifts in voices.
%  Related to (a): Prior work in AI-mediated communication suggests AI suggestions can shift writing tones, styles, and topics.
%  Related to (b): Prior work in writer-reader relationships suggests readers have the expectation for writers to put in their own work, and writers have the desire for genuine expressions.

% [Control over AI writing assistance] 
% Writers’ perceived control in the writing process shapes their perceived ownership of work.
% Meanwhile, agency of AI co-creation applications affects whether users perceive AI as tools (and have control over them) vs. as collaborative partners.


% Highlight literature gaps
Together, these emerging themes suggest that on the one hand, writers have growing concerns about AI's potential threats to authentic writing.
On the other hand, \textit{\textbf{it is unclear whether and how writers' authentic voices in writing can be preserved.}}
%Besides, these prior studies mostly focus on relevant yet specific aspects of authenticity only.
Prior work also tends to focus only on specific aspects of authenticity.
For instance, studying authorship specifically addresses the \textit{source} component of authenticity, while examining the impact of AI assistance on writing outcomes resonates with the \textit{category} approach.
As a result, we lack a more holistic, writer-centered view of authenticity in human-AI co-writing.
Without comprehensive perspectives from writers, it remains difficult to propose ground-up, effective solutions to regain and protect authenticity in their co-created work with AI.
Our present research aims to address these literature gaps and design goals.


% \placeholder{Besides unresolved questions stemming from these studies, prior literature tends to focus on specific aspects that are partially relevant to authenticity. For instance, studying authorship specifically addresses the \textit{source} component of authenticity, while examining the impact of AI assistance on writing outcomes resonates with the \textit{category} approach. However, there lacks a more holistic view toward authenticity and the meaning of authentic work in human-AI co-creation. Among many of the above-mentioned studies, concerns for authenticity came out from writers, but research directly examining the subject of authenticity is scarce. Finally, despite growing concerns around this topic, \textbf{it remains unclear whether and how writers want to preserve authenticity in human-AI co-creation.} Without a clearer understanding of what authenticity is, it remains difficult to act toward addressing these concerns.}


\subsubsection{Insights from AI-mediated communication research}
Prior research on AI-mediated communication (AIMC) might bring additional perspectives on these unresolved questions around authenticity. More abundant AIMC studies have looked at how AI suggestions mediate written content for communication through text, including readers' perceptions of both the content and the message writer~\cite{AIMC_Hancock_JCMC_2020, AIMC_positivity_social_attraction, AIMC_topic_choice_self_presentation, AIMC_social_relationship, AIMC-perceptions-of-generated-problematic-replies}.
Meanwhile, writing can also be viewed as a medium of communication that connects the writers and their audiences, albeit often not bi-directional or at the inter-personal level~\cite{writer-reader_Candlin_Hyland_1999, writer-reader_sharing_words, writer-reader_writing_for_readers}.


% evidence that AI assistance could mediate content output --> shift authentic voices in writing
Indeed, various AIMC research shows AI assistance (e.g., word-by-word suggestions or short-reply suggestions) could shift the characteristics of writing content, such as a more positive tone~\cite{AIMC_positivity_social_attraction, AIMC_Hancock_JCMC_2020, AIMC-perceptions-of-generated-problematic-replies}, or even affect topics addressed in writing~\cite{AIMC_topic_choice_self_presentation}.
More recently, \cite{HAIC_authenticity_Opinionated_LLM} found that writing with AI assistance on opinionated content not only affects a user's writing output but also their own opinions toward the written topic.
Together with repeated findings around readers' negative perceptions of communicators who use AI~\cite{jakesch2019ai,liu2022will}, scholars expressed ethical concerns around AI's implications on information and interpersonal trust~\cite{AIMC_email_trust, AIMC_uncertainty_source}, user's sense of agency and authenticity~\cite{AIMC-perceptions-of-generated-problematic-replies}, and social relationships~\cite{AIMC_social_relationship, AIMC_positivity_social_attraction, AIMC_profile_airbnb} as users more widely adopt AI for composing content for interpersonal communication.


These findings suggest AI's potential to move writers away from their own voices in writing,
% Furthermore, AI mediation may affect writers' opinions and attitudes during their writing processes \tocite{},
though it is not clear whether insights from AIMC research apply to understanding AI-assisted writing more generally.
Once again, we know little about how writers could avoid compromising their own voices when writing with AI.
Additionally, the unique connection between professional writers and their readers through writing is also often different than the forms of interpersonal communication researched in the context of AIMC.
Prior AIMC work often examines content written in mutual conversations for instrumental purposes (e.g., communicating with an owner of a rental house) or relationship building (e.g., emailing a friend)~\cite{AIMC_profile_airbnb, AIMC_Hancock_JCMC_2020,liu2022will}.
Unlike such dialogues, writers seldom speak to a particular individual nor aim to build interpersonal relationships with their audiences.
Instead, writers use writing as a means to deliver their messages to a crowd and express themselves creatively.
We thus investigate how these differences add to the complexity of authenticity in human-AI co-writing.


% Vera's comments:
% I still wonder whether AI mediated communication should be a separate literature review section (also refer back in discussions). Perhaps we should take the position that readership is a form of communication but may differ from relational and transactional inter-personal communications?? Some possible relevant points:

% ethical considerations as genAI is used to communicate/produce information: e.g. implications for /harms inter-personal relationship/trust: https://academic.oup.com/jcmc/article/25/1/89/5714020; also relevant: “uncertainty” in communication and information ecosystem: https://arxiv.org/abs/2311.01193 (uncertain about information is produced by whom, when, where and why)

% open questions regarding how people actually perceive AI-assisted communication, and (somewhat mixed) empirical results: most papers found that once receipients know it is AI generated, they perceive the sender negatively (digging up papers from Maurice Jakesch, Hannah Mieczkowski etc https://dl.acm.org/doi/abs/10.1145/3544548.3581196, https://dl.acm.org/doi/abs/10.1145/3290605.3300469.). But I think this paper has some mixed results: https://dl.acm.org/doi/abs/10.1145/3491102.3517731. But the prior literatures are all/mostly about transactional/instrumental (e.g. airbnb) communication or relational (e.g. email)

% (not sure if this point goes here or “shifting genuine voice” many papers also studied how ai-mediation shift content characteristics (e.g. more positive sounding https://academic.oup.com/jcmc/article/25/1/89/5714020). 
% Reduce content diversity: https://arxiv.org/abs/2309.05196; 
% shift opinion/latent persuasion in both produced content and writers’ actual opinion: https://dl.acm.org/doi/abs/10.1145/3544548.3581196; 
% affect topic choice https://dl.acm.org/doi/abs/10.1145/3544549.3585893


%\textit{RQ2: Whether and how does authenticity matter to writers when co-writing with AI?}

%\textit{RQ3: Whether and how does co-writing with AI affect writers' authentic voices in writing? (RQ3a) If so, how do writers preserve authenticity when co-writing with AI? (RQ3b)} % Does AI shift writers away from their authentic voices in writing?

% \textit{RQ4: What other concerns do writers hold toward co-writing with AI?}


\subsection{Designing Tools for Human-AI Co-Writing}

Recent work has already revealed a wide variety of possible AI writing assistance scenarios (see our summary in Table~\ref{tab:AI_writing}), ranging from more generic to genre-specific support. 
Researchers have also experimented with AI assistance that supports different stages of one's writing process as well as providing multi-form~\cite{AIwriting_Tool_wordcraft, AIwriting_tool_wordcraft_creative_writing}, multimodal~\cite{AIwriting_Tool_integrative_leap_multimodal} support at once.
While many of these explorations were shown to be helpful for writers, the majority of these studies focus on improving usability, productivity, and sometimes creativity of writing. 
By contrast, the possible influences of these tools on authenticity often only arise in exploratory analyses or post-study conversations with participants, leaving a noticeable literature gap.

% Other papers on AI-assisted writing tool:
% https://dl.acm.org/doi/abs/10.1145/3490099.3511105
% https://dl.acm.org/doi/abs/10.1145/3544548.3581225
% https://dl.acm.org/doi/full/10.1145/3511599 (also proposed the concept of “integrative leaps” when working with AI)
% https://dl.acm.org/doi/abs/10.1145/3290605.3300526
% https://dl.acm.org/doi/abs/10.1145/3532106.3533533
% https://dl.acm.org/doi/abs/10.1145/3526113.3545672


% We explore this topic through personalized vs. non-personalized tools.
% \textit{RQ5: What types of support do writers seek in creative writing with AI?}


\input{table/table_AI_writing}



% \subsection{Personalized Support in Human-AI Co-creation}
% \textit{RQ6: Whether and how do personalizing co-writing experiences with AI affect authenticity in writing?}


\section{Methods}

\subsection{Overview of the Study Design}
We examined writer-centered definitions of authenticity and the impact of AI and personalized AI writing assistance on authentic writing primarily through semi-structured, qualitative interviews with professional writers. 
To enable participants to respond to these inquiries with situated experiences, we adopted two versions of AI-powered writing assistance tools: one with personalization through in-context learning, and one without personalization. 
We investigated how participants wrote with generative AI in real time and delved into their co-writing experiences through interviews following each writing session. 
We complemented perspectives from these direct users of the emerging technology (i.e., {\em writers}) through a follow-up online study with indirect stakeholders (i.e., {\em readers}) \cite{Friedman_value_sensitive_design}. 
Through these two parts of the study, we synthesize a more comprehensive view of authenticity in writing.
The full study protocol was reviewed and approved by the Institutional Review Board (IRB) of the authors' affiliation.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/Screenshot 2024-01-17 at 6.58.38 AM.png}
    \caption{Study procedure of Part 1 and Part 2}
    \label{fig:enter-label}
\end{figure}


\subsection{Part 1: Interviews with Professional Writers}
We conducted Part 1 of the study with 19 professional writers.
The study includes a pre-interview survey (done through an online questionnaire) where participants shared their writing samples and professional experiences as writers and expressed their opinions on what authenticity in writing means to them and on AI writing assistance.
During each interview, we first asked participants to further elaborate on their perspectives regarding authenticity and co-writing with AI.
Next, participants engaged in two writing sessions to co-write a short passage with a personalized and a non-personalized AI writing assistance tool in a randomized order.
Immediately after each writing session, we asked participants to reflect on their co-writing experiences through semi-structured interviews.
After both writing sessions, we asked participants to compare their experiences across the two sessions.
Finally, we revealed to them the difference between the two tools and asked them a few more questions to capture their overall thoughts on co-writing with generative AI.
The pre-study survey and the full interview protocol are included in Appendix~\ref{appendix:pre-survey} and \ref{appendix:interview_protocol}.

% \todo{add a study flow chart}


\subsubsection{Recruitment and participants}
We recruited 21 professional writers through Upwork, a platform frequently used to recruit professionals with specific expertise. 
We partnered with a recruitment specialist from the Upwork team to ensure candidates provided authentic information on their profiles and verified their past freelanced work on the platform.
We also used the pre-interview survey for screening purpose, in which participants elaborated on their professional experiences as writers, shared their writing samples, and provided relevant links to their professional websites and profiles (See more details of the pre-interview survey in Section~\ref{sec:writer_pre-survey}).
One of the participants did not show up and one decided to drop out from the study, resulting in N = 19 participants who fully completed the study; data from all 19 participants was used for analyses.


\input{table/table_writer}


\subsubsection{Pre-interview survey}
\label{sec:writer_pre-survey}
The pre-interview survey begins with obtaining informed consent from participants (by signing a consent form).
After consenting, participants responded to a series of questions through free text responses.
These questions ask participants to describe (1) the unique characteristics of their writing, (2) their prior experience working with AI and non-AI writing tools, if any, (3) their definition of authenticity in writing.
At the end of the survey, participants were asked to submit a short writing sample of their own (~ 200 words) that represents their work. Participants were informed their writing samples would be used as to design the study task for them (if selected to participate), though we did not specify how so.
We asked participants to select work that best represents their authentic writing.
We use the writing samples for in-context learning to prepare a personalized AI writing assistance tool for the interview session (see more details in the next section).


\subsubsection{AI writing assistance}
We adopted open-source code from \cite{Mina_Lee_CoAuthor} to run the CoAuthor interface with GPT-4 and used it as the AI writing assistance tool for the interview sessions (see Figure~\ref{fig:coauthor} for the CoAuthor interface). CoAuthor is a system built by Lee et al. \cite{Mina_Lee_CoAuthor} that allows writers to request next-sentence suggestions from an LLM, and the open-source code allows for customization, such as choosing which LLM to use and its parameters. % \VL{the paper never includes an interface...should we add?}
We chose CoAuthor as the writing assistance tool for this study for two reasons: 
(1) As we targeted writers with expertise in a diverse set of writing genres, we chose a tool that was \textit{not} designed to support a particular type of writing. 
(2) Since participants had a limited time to become familiar with the AI writing assistance, we avoided more complex tools with multiple forms of support (e.g., Wordcraft~\cite{AIwriting_Tool_wordcraft}).
%(3) Though CoAuthor only supports a single type of writing assistance (i.e., sentence-level suggestions), it goes beyond word-by-word completion so that we can better differentiate the findings of the present work from those revealed in prior AIMC research. 
%\VL{AIMC works also studied sentence suggestion, and if you mention this, should we attribute our results difference just to the sentence level suggestions? I worry mentioning this might hurt the paper}
%\angel{right, this last point could be misleading - commenting it out now}


\begin{figure}
    \centering
    \includegraphics[width = 0.6\textwidth]{fig/coauthor_UI.png}
    \caption{Interface of the CoAuthor system (image adopted from \cite{Mina_Lee_CoAuthor}), which contains a text editor where users can request (Tab key) and adopt AI (Enter key) suggestions through keyboard shortcuts.}
    \label{fig:coauthor}
\end{figure}


Before each session, we used the writer's submitted writing sample as data for in-context learning to create a personalized version of the CoAuthor tool for their session.
We used the following parameters for GPT-4 to generate suggestions: max tokens = 5; temperature = 0.9; top p = 1; presence penalty = 0.5; frequency penalty = 0.5.
During the co-writing sessions, writers were able to request AI writing suggestions at any time by the Tab key.
The tool would generate around 5 sentence-level suggestions based on the written text.
Writers could accept, reject, and revise the suggestions as they like.
At the beginning of their first writing session, the researcher who led the study session walked the writers through the CoAuthor interface and guided them to practice using the tool to write a few sentences. 
This was to ensure participants fully understood and became familiar with the tool before they started their first formal writing session.


\subsubsection{Co-writing session with AI}

Participant were asked to write one short passage (around 200 words) for each co-writing session on a topic similar (but not identical) to that of their submitted writing sample. %\todo{add writing topic to participant table}
Each co-writing session lasted between 20 - 25 minutes. The time was determined by piloting with two professional writers.
All participants were able to finish their assigned 200-word passage within the time frame.
As participants wrote, we used the CoAuthor interface to record their writing logs and their final writing output.
Writers' behavioral data recorded through the writing logs include (1) the frequency and timing of their requesting AI suggestions, (2) the frequency and timing of them accepting and/or rejecting AI suggestions, (3) the AI suggestions (in text) provided at each of their request, (4) the AI suggestions (in text) accepted, if any, and (5) the text inserted by writers. 
Additional details about the writing logs can be found in Appendix~\ref{appendix:writing_log}.


\subsection{Part 2: Online Surveys with Regular Readers}
In Part~2, we conducted an online study to understand frequent readers' perceptions of authenticity, AI writing assistance, and work co-written by human writers and AI.
We used writing work produced by six writers in Part~1, each of which represents a unique literature genre (P8: science fiction/fantasy, P10: biography, P12: poetry, P14: spiritual, P15: romance, and P19: screenplay), as materials for Part~2.\footnote{At the end of each session in Part 1, we informed writers and obtained their consent to use their writing for subsequent research.}
These include anonymized writing samples that writers submitted in the pre-interview survey of Part~1 (i.e., work written by themselves) as well as the two passages they wrote with the personalized and non-personalized AI during Part~1.

Participants of Part 2 (i.e., Readers) first responded to a few open-ended questions about their attitudes toward AI-assisted writing.
They then read and assessed three writing passages from the same writer (their solo work, work with personalized AI, and work with \revision{non-}personalized AI) by likeability, enjoyment, and creativity.

Next, readers performed two sets of comparisons with the three pieces of writing.
First, they were asked to compare and rate how likely each piece was written by a human writer alone or with the help of an AI writing support tool (while only being informed that \textit{some} of these pieces were written with AI).
%Readers were informed the three pieces of writing were either written independently by a human writer or co-written by the same human writer and an AI writing assistance tool. 
Second, readers were informed which piece was the writer's solo work.
They then compared the two AI-assisted writings, rating how much they sound similar to or different from the writer's voice in the solo writing. 
They were also asked to identify which part(s) of the writing might adopt AI assistance.
Readers were blinded to the two different AI conditions; namely, they did not know which one was co-written with a personalized versus a non-personalized AI tool, nor personalization was the variable being studied.
%They also did not know personalization was the manipulated variable in Part~1.

After rating and comparing writing passages, participants responded to a few questions about their general perceptions of AI-assisted writing.
The full Part~2 questionnaire is attached in Appendix~\ref{appendix:part2_survey} and descriptive statistics of numeric measures were reported in Table~\ref{tab:descriptive} (columns for multiple rounds will be explained below).
The entire Part~2 study was conducted online and took around 45 - 60 minutes to complete.
Participants received cash compensation for their participation.
Once again, the study protocol was reviewed and approved by the IRB of the authors' affiliation.


\input{table/table_part2_descriptives}


\subsubsection{Recruitment and participants}
We recruited participants on Reddit to find highly involved readers who regularly read the particular literature genres written by those six writers chosen from Part~1.
One of the researchers joined multiple subreddits dedicated to discussions about reading.\footnote{We received approvals from community moderators to post and participate in the discussion on these subreddits.} (See Appendix~\ref{appendix:subreddit} for these groups.)
%Many of these Subreddits also focus on specific literature genres.
Recruitment messages were posted on discussion threads in these subreddits.
Interested individuals first filled out an interest form that surveyed the literature genres and frequency they read. They also reported the subreddit where they saw the recruitment message.
We recruited participants who read their interested genres at least once a week.
As prior research on Reddit identified a large number of machine-generated responses, we showed some question texts in an image format in the interest form to filter out bots that can only read texts.
We also included an open-ended question (i.e., ``In one to two sentences, describe your favorite literature genre and why you favor it.'').
Two researchers reviewed these open-text responses and screened out those that were likely generated by machines, as detailed below.


%\subsubsection{Study questionnaire}
%\label{sec:part2_survey}




\subsubsection{Screening AI-generated responses}
We first set out to collect feedback from three readers for each writer's work, resulting in $6\times3 = 18$ participants.
However, we noticed a substantial number of open-text responses that might be AI-generated (e.g., by ChatGPT) after examining our initial batch of data.
We discussed among our research team to consolidate the following criteria for screening: (1) Responses were consistently written in a bullet-point style following the structure of "[Topic]: [Description]", which is a common style in ChatGPT output; (2) We used our survey questions as prompts and collected responses from popular generative AI tools, including ChatGPT, Microsoft Bing, and Google Bard. We cross-checked whether participants' responses overlapped significantly with those AI-generated ones.

Two researchers independently read through these responses and marked responses that were likely AI-generated. 
Any disagreement was reviewed by a third researcher.
In the end, we marked 7 participants who likely used AI to generate open-text responses throughout the study.
We thus conducted a second round of data collection and applied the same screening criteria to attain a larger sample size with sufficient power for data analysis. 
We targeted having at least 5 readers rating each passage; 
the final sample size after Round 2 of data collection is N = 30.
For all analyses, we reported results using data from both rounds of data collection. 



\section{Results}

\subsection{Overview of Data Analysis}
We conducted analyses with three streams of data: a)~the interview data and b)~writing logs (i.e., behavioral data) from writers in Part~1, and c)~survey data with readers in Part~2.
We transcribed the interview data and analyzed them through thematic coding and affinity diagrams.
While the first author led the qualitative data analysis, the research team met weekly to discuss findings in order to reduce subjectivity during the data analysis phase
(See Appendix~\ref{appendix:codebook} for the full codebook). 
%We used R to perform quantitative data analyses.
For any within-subject comparison (e.g. writers' behavioral logs using the two versions of AI tool), we used 
%the \verb|lmer| package to run 
linear mixed effect models, controlling for participants' subject IDs and order effect.\footnote{To run the linear mixed effect models, we used the $|lmer|$ R package.}
For scales that capture individuals' opinions toward AI-assisted writing (e.g. readers' survey responses), we used Chi-squared tests to examine whether participants' ratings differ significantly by ordinal levels.\footnote{We used Chi-squared tests instead of normality tests for distribution as each of these variables was measured by a single 5-point scale. Thus, we treated the data as ordinal instead of continuous numeric values.}
Details for our analytic approaches are listed in Table~\ref{tab:stats_model}.
We organize our results according to our research questions with data from different streams, when applicable. We also present two additional points emerged from our interviews with writers:
\begin{itemize}
    \item In Section~\ref{sec:def_auth}, we first address writer-centered definitions of authenticity in writing and the impact of co-writing with AI on authenticity (RQ1).
    \item In Section~\ref{sec:writing_practice}, we elaborate on how writers would like to preserve their authentic voices through practices of writing with AI (RQ2).
    \item In Section~\ref{sec:personalization}, we compare whether and how personalization of AI writing assistance affects writers and readers' experience, respectively (RQ3).
    \item As discussions around writer-reader relationships as well as alternative forms of writing support emerged frequently in our interviews with writers, we further elaborate on them in Section~\ref{sec:writer_reader_relationship} and Section~\ref{sec:future_support}, respectively.
\end{itemize}


\input{table/table_stats_model}


\subsection{Writer-Centered Conceptions of Authenticity in Writing}
\label{sec:def_auth}

Our findings first reveal how writers conceptualized authenticity through \textit{the source of content}, \textit{internal experiences and identities} that ground writers' work, and the actual \textit{writing outcomes}. 
Although writers' reflections did resonate with some of the definitions of authenticity as established in the existing literature (i.e., category, source, and value), they placed further emphasis on viewing authenticity through writers' internal experiences instead of through their explicit expressions in writing.
Moreover, regardless of how writers defined and understood authenticity, many of them indicated authentic writing \textit{is} the essence of good writing, and saw the likely impact of AI on authenticity in writing.


\subsubsection{Defining authenticity through the source of content (Source authenticity)}
% This point is related to the construct of “source” as in prior literature
% Impact of co-writing with AI on authenticity: When AI participates in writing, writers are no longer the sole source of content generation, leading questions to authenticity in writing.

Several writers described authenticity as a \textit{``who''} question, focusing on the source of content production.
This concept mirrors \textit{source}, a long-standing theoretical component of authenticity in the existing literature, and is directly related to considerations for authorship.
Writers who held this view also saw AI writing assistance as a direct threat to authenticity.
With AI participating in the writing process, writers are no longer the sole source of content generation, raising questions about the authenticity of their writing.


%\subsubsection{Defining authenticity through the process and writers' internal experiences of constructing and expressing their authentic self}
\subsubsection{Defining authenticity through constructing and expressing their authentic self}
% expanding beyond just alignment

Writers mentioned several internal states during their writing processes as key constructs of authenticity, many of which have been less covered by prior literature. 
%not yet been thoroughly discussed in the existing literature.
These include (1) whether writers can freely express their emotions to form emotional connections with their readers, (2) whether the process of writing allows them to feel passionate about their work, (3) whether they have the autonomy to select topics and content that are personally important to them, (4) and most importantly, whether a writer can justify having their name and identity behind their work.
In other words, a writer claims the authenticity of their writing if they can soundly argue why the piece of work can only be done by them as \textit{the} author.

This view of authenticity is shaped by the belief that writers’ identities, backgrounds, and lived experiences serve as fundamental materials of writing and enrich their work.
Building on such cornerstones, whether writers can genuinely express their own experiences and identities through the writing as well as whether they feel enthusiastic and believe in the importance of
%would feel importance and enthusiasm for 
their work---due to these personal values that are attached to their work---jointly contribute to authenticity.
As such, the work would never be in its current form if produced by any other writer.
One writer described it metaphorically:

\begin{quote}
    I've often said that writing is a lot like a tree. The trunk of the tree is the idea. Everybody can have the same idea and then start to write something. But eventually, once you get up into the branches, everybody's going to go off in their own different branch. Authenticity is your own personal branch, the way that you would take an idea and how it would be different from 50 other people who take the same idea and try to finish it or complete it to the end. (P19)
\end{quote}


However, when AI contributes to writing, the content is no longer grounded solely on writers’ own experiences, memories, backgrounds, knowledge, research, and more.
Although it is not always clear to them what else the work is established on, writers can no longer claim their work as a reflection of their lived experiences or even an epitome of themselves.


\subsubsection{Defining authenticity through writing outcomes (Content authenticity)}
% This point is related to the construct of “category” as in prior literature, but it is also the least prominent for writers
% Impact of co-writing with AI on authenticity: AI’s influences might shift writing output from the “typical” ways in how writers write.

Examining the outcomes of writing is yet another approach to assessing authenticity.
More specifically, authentic writing equals writing that best represents the work of a writer, where one can tell who the author is by reading the text.
This perspective echoes the ``category'' construct of authenticity, which is the most adopted definition of authenticity in the literature space~\cite{Auth_Humanity_Guignon_2008, Auth_Humanity_AMA_Lehman_2019, Auth_Humanity_Handler_1986}.
Nonetheless, it was the least referred to and a less critical construct from writers' points of view.
Among the few writers who defined authenticity through this lens, they were concerned about the influences of AI writing assistance on authenticity, as AI's input might ``shift writers away from the typical ways of [their] writing practices'' (P2), intruding on the authentic voices in their writing.
Under this conception of authenticity, since writers evaluate authentic writing by comparing it to one's representative work, they also connected the meaning of authenticity back to various writing elements (e.g., word choice, style, use of references and metaphors) that uniquely characterize their own writing.


\subsection{(Re)claiming Authenticity Through Practices of Co-writing with AI}
\label{sec:writing_practice}

Through the co-writing sessions, writers identified several practices during the writing process that could help shape authenticity in writing with AI assistance.
In other words, \textit{how} writers use AI while writing plays a key role in determining the authenticity of AI-assisted writing. 
These determinants include: (1) whether one starts with an clear vision for writing in mind, (2) when one calls for writing assistance from AI, (3) what portion of contribution one makes in the writing, and (4) what purpose and usage that AI writing assistance serves.


%\subsubsection{Is there an image at the starting point?}
\subsubsection{Setting off with a clear image for writing}
% whether writers had a clear idea or a clear image of what they want and how they want to present themselves in writing

In describing their writing, writers reported that they seldom start writing with a blank sheet.
Instead, they typically begin their processes with some vision for writing in mind.
Such a vision need not be a concrete, fully fleshed-out idea. 
But writers would already have certain directions or atmosphere that they would like to set up for the passage, given the preparation work they did before writing (e.g., ideation, research, collecting references and other writing materials). 
Otherwise, they lack an anchor to guide how they cohesively respond to, select, and curate AI suggestions alongside their own streams of writing.
In such case, they might be at more risk of being affected by AI suggestions, depriving their authentic voices in writing.


\begin{quote}
    I think it [AI] has the possibility to [affect writers] if you let it. But if you already have your ideas of what you want to stay true to, then it isn't going to affect your authentic voice, in my opinion. So to me, it comes down to user influence and how much the user chooses the directions that the AI suggests. (P4)
\end{quote}


%\subsubsection{When did writers use AI during their writing processes?}
\subsubsection{Working with AI through the ``fuzzy area'' of idea development}
% there is a fuzzy area in the writing process, where one already has a broad idea/direction for writing but it hasn't been externalized, shaped, and refined into an actual piece of writing
% this is where AI has the most potential to support writing without compromising authenticity

It is worth recognizing that writers work through various stages throughout their writing processes.
While writers bring a premature vision to initiate writing, there is typically a ``fuzzy area'' (P04) between the starting point and well-developed ideas, which eventually leads to a fully crafted piece of writing.
AI writing assistance is most acceptable and is considered as having the least harm on authenticity at this middle ground for two reasons.
First, the ways in which writers would interact with AI writing assistance tools during this stage primarily serve to consolidate and further develop their ideas (see more details in Section~\ref{sec:AI_usage}).
Here, writers write to incubate and organize their thinking instead of producing text to construct the actual piece of writing.
Therefore, though AI suggestions contribute pieces of content, they serve as materials that facilitate the thought processes rather than the writing \textit{per se}.


% \subsubsection{Who did more work for a piece of writing?}
\subsubsection{Claiming contribution through content gatekeeping}
% Evaluating portions of contributions
% Human writers as content gatekeepers

Most importantly, writers considered AI-assisted writing as authentic as long as they contributed more to the writing.
Specifically, writers noted one's \textit{contribution} does not necessarily equal how much text they wrote. %distinguished the portion of \text{contribution} from the actual length of text written. 
In their view, real contributions require ``content gatekeeping'' (P8)---that is, actively deciding what goes into the writing content.
Given this conception of contribution, writers commonly believe they did most of the work during the writing process as they took charge of selecting, revising, and incorporating AI suggestions into their writing.
Whether a word, a sentence, or a paragraph is produced with AI assistance or not, it is the human writer, instead of the AI tool, that takes control over whether to adopt, remove, or revise each piece of content.


% \subsubsection{What did writers use AI for?}
\subsubsection{Beyond AI as a co-writer: Opportunities for supporting authentic writing processes} %\VL{I am struggling a bit with what this section is about...the content does not always suggest concrete "co-writing forms'', and they are not "beyond writing". I first tried to revise the title as ``beyond content suggestions'', but I saw at least the first two points are still about content suggestion somewhat...I feel they are "(high-level) conceptualization of how AI can contribute to (authentic) writing process'' or ``AI opportunities for authentic writing processes''...} \angel{so kind of close to the idea of "beyond writing"... this group here says about how AI can help to preserve writers' authentic voices in writing but *not* by doing the writing job, especially not doing the job of producing a full piece of text.} \VL{When you say ``beyond writing'', it is not clear this is about ``AI doing the writing'', what about ``beyond AI as a co-writer/coauthor: opportunities for supporting authentic writing processes''?}
\label{sec:AI_usage}
% AI as internalization tool
% AI as jumping points and driving forces that keep the writing flow going
% AI as sounding board

Besides requesting content suggestions from AI (i.e. what the CoAuthor interface supports), writers believe they could benefit from AI assistance while preserving their authentic voices by leveraging AI capabilities as  \textit{means of internalization}, \textit{a driver of the writing flow}, and \textit{a sounding board of public feedback}. Below, we unpack each of these favorable co-writing forms that our participants indicated:


\textbf{\textit{AI as means of internalization:}}
Nurturing themselves through reading, researching, and experiencing the world is key to the quality and richness of writers' work.
Writers often improve their work over time by reading and getting inspired by others' work.
Thus, they saw AI as a means to help them absorb large amounts of information and saw AI suggestions as excerpts resulting from this practice.
As P18 described: 

\begin{quote}
    ``The way that we actually improve ourselves is by reading other people's works. Our memory retention on how other people worded things is in the background of our minds when we need to write something of a similar nature. [...] But really what you're doing is regurgitating what you've read maybe 20 years ago, ten years ago, or just five or 4 hours ago, doing it in your own unique way and telling your own unique story. % Stephen King even promotes the idea of reading for 4 hours a day and writing for 4 hours a day. 
    [...] This [AI writing assistance] is kind of combining those two things [reading and writing] all at once. So instead of reading, I'm getting an option which is exactly what the reading is supposed to do for you. And I can choose that option or choose to go with my own authenticity, my own way of actually writing it.''
\end{quote}

Under this notion, some participants saw an analogy with how AI is built (i.e., learning from large amounts of text to produce text). 
Namely, like how human writers consume loads of information and experiences to enrich their writing, AI digests vast amounts of data to generate text --- though the machine expedites this process significantly.
In other words, while writers gradually take in their work and life experiences to enrich their writing, they see AI as a potential tool that compresses this process and presents the results of internalization.
As P10 put it in a critical way, ``if what this AI does for the writer is unauthentic, then, perhaps there is no such thing as authentic writing.''


\textbf{\textit{AI as a driver of the writing flow:}}
Having the option to continuously request assistance from AI may help carry on writers' writing flow and remove writing blocks.
Occasionally, AI suggestions might point to novel directions or ideas that writers would not have conceived by themselves, and the tool could also offer ``jumping points'' that allow writers to transition from one idea to another. 
However, these benefits are secondary to AI's capability of ``keeping [writers] up with their momentum'' (P08).
It not only takes warm-up time for writers to immerse themselves in a smooth writing flow, but once the flow experience is interrupted, it could be difficult to resume.
Writers saw AI suggestions as on-demand, temporary remedies when they sense an emerging rift in their writing process.


\textbf{\textit{AI as a sounding board of public feedback:}}
Several writers were aware large language models are trained with vast amounts of text data from the Internet and across digital outlets.
As such, they viewed these models as an assembly of information and opinions online, and would like to use it as a sounding board to potentially project and reflect responses from broader audiences.
Writers saw AI suggestions as syntheses of the public's interests, and they were interested in using such information to navigate and/or improve their own work.


\subsection{Finding and Preserving Authentic Voice: Personalization as Double-Edged Sword}
\label{sec:personalization}
We discuss how writers perceived the impact of personalized AI on their writing, together with whether and how personalization affected their usage behaviors with the tool, and how readers responded to their writings with personalized versus non-personalized AI assistance based on data from the reader survey.

\input{table/table_part2_analysis}

\subsubsection{Writers' subjective preferences toward personalized AI}
Comparing their experiences co-writing with the personalized AI and the non-personalized AI, writers reflected on both the positive and negative impact of personalization on authentic writing after we revealed that one of the tools they experienced was powered by a personalized LLM with the writing sample they provided.
Overall, the majority of writers preferred working with personalized writing tools when they were asked to compare the two options.
This is because writers believed personalization could help preserve their genuine voice, express themselves naturally, and better connect with their own identities.
But at the same time, personalization might also lead to writers adopting more suggestions from AI, allowing more influences from the tool.


\subsubsection{Writers' adopted a similar degree of assistance from both personalized and non-personalized AI tools}
Despite writers' subjective preferences for the personalized tool, in our study there is no significant difference in the frequency of requesting AI assistance when working with the personalized vs. the non-personalized tool ($\beta = 0.13$, $S.E. = 1.08$, $t = 0.12$, $p = 0.904$).
Likewise, writers' behavioral data from the writing logs shows no significant difference in the rate of accepting suggestions from AI between the personalized vs. non-personalized condition ($\beta = -0.02$, $S.E. = 0.07$, $t = -0.27$, $p = 0.790$). (Also see Appendix~\ref{appendix:writing_log} for the statistics reported by each writer.)

\begin{comment}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{fig/part1_get.png}
    \caption{Number of times each writer participant pulled up AI assistance when writing with the personalized vs. non-personalized tools.}
    \label{fig:part1_get}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{fig/part1_accept_rate.png}
    \caption{Rate (\%) of AI suggestions accepted by each writer participant when writing with the personalized vs. non-personalized tools.}
    \label{fig:enter-label}
\end{figure}    
\end{comment}


\subsubsection{Readers' responses to personalized and non-personalized AI-assisted writing}
%From readers' perspectives, they 
The readers in the second part of our study expressed similar experiences reading the three types of passage---writers' solo work, the work they produced with personalized AI, and the work with non-personalized AI.
Per readers' numeric ratings, the degree of enjoyment ($F = 0.63$, $p = 0.536$), likeability ($F = 1.23$, $p = 0.298$), and creativity ($F = 1.19$, $p = 0.311$) after reading each type of passage shows no significant difference across the three conditions. Pair-wise comparison also shows no significant difference (See Table~\ref{tab:part2_analysis} for statistics). Furthermore, readers were not able to precisely identify which part of the text contained AI-assisted output, and this rate of correct identification has no significant difference between the personalized and non-personalized conditions.

When asked to compare across the three writing passages, reader participants rated the solo human work as more likely to be done independently by a human writer than the two forms of AI-assisted writing (solo $-$ personalized AI: $\beta = -0.73$, $S.E. = 0.25$, $t = -2.94$, $p = 0.004$; solo $-$ non-personalized AI: $\beta = -0.64$, $S.E. = 0.24$, $t = -2.57$, $p = 0.011$), while there is no significant difference between the work co-written with the personalized vs. non-personalized AI ($\beta = 0.09$, $S.E. = 0.26$, $t = 0.35$, $p = 0.727$).
When comparing the two AI-assisted writing pieces to each writer's solo work, readers did not notice any difference regarding whether the AI-assisted work preserved the writer's authentic voice ($\beta = 0.07$, $S.E. = 0.21$, $t = 0.36$, $p = 0.722$). 


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.55\textwidth]{fig/part2_rating_condition.png}
    \caption{Reader participants' ratings to compare the three pieces of writing. Left: Ratings for whether a piece of writing is likely to be done independently by a human writer (rating = 5) or co-written with AI (rating = 1) on a 5-point Likert scale. Right: Ratings for whether a piece of AI-assisted writing preserves a writer's authentic voice.}
    \label{fig:part2_rating}
\end{figure}


\begin{comment}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{fig/part2_bar_combined.png}
    \caption{Reader participants' ratings for whether a piece of writing is likely to be done independently by a human writer (rating = 5) or co-written with AI (rating = 1) on a 5-point Likert scale.}
    \label{fig:prob_human}
\end{figure}
\end{comment}


\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{fig/part2_rating_by_author.png}
    \caption{Reader participants' ratings for writing passages for each writer. Left: Ratings for whether a piece of writing is likely to be done independently by a human writer (rating = 5) or co-written with AI (rating = 1) on a 5-point Likert scale. Right: Ratings for whether a piece of AI-assisted writing preserves a writer's authentic voice.}
    \label{fig:part2_prob_human}
\end{figure}


We took a closer look at readers' ratings for writing from each of the six writers respectively. For 4 out of the 6 writers, work co-written with non-personalized AI was perceived as more likely done by a human writer independently. The two writers (P14 and P15) whose work was rated as more human-like when working with the personalized AI wrote about romance and spiritual topics respectively. We cross-checked the ratings from the readers with the writers' behavioral data, and we found these two writers also accepted more suggestions from the personalized AI than from the non-personalized during the writing sessions (P14 accepted 67\% of suggestions from the personalized AI vs. 41\% from the non-personalized AI; P15 accepted 71\% suggestions from the personalized AI vs. 20\% from the non-personalized AI).

We note that recent research reports that people could not reliably distinguish whether a piece of content is generated by people or the latest LLMs~\cite{jakesch2023human}. While our results suggest that readers might be able to tell if a piece is co-written with AI with some degree of confidence, they may not respond significantly differently to content written by the writer alone or co-written with AI in terms of how much they enjoy reading it, at least in the kind of leisurely reading context we studied (i.e. the reader did not have frequent exposure to or actively seek out the writer's work).

\begin{comment}
    \begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{fig/part2_prob_human_author.png}
    \caption{Reader participants' ratings for whether a piece of writing is likely to be done independently by a human writer (rating = 5) or co-written with AI (rating = 1) on a 5-point Likert scale.}
    \label{fig:part2_prob_human}
    \end{figure}
\end{comment}


\begin{comment}
    \begin{figure}[h!]
    \centering
    \includegraphics[height=0.35\textwidth]{fig/part2_cowriting_auth_author.png}
    \caption{Reader participants' ratings for whether a piece of AI-assisted writing preserves a writer's authentic voice.}
    \label{fig:part2_prob_human}
    \end{figure}
\end{comment}


\subsection{About Time: Rethinking Writer-Reader Relationships in the Age of Generative AI}
\label{sec:writer_reader_relationship}

\subsubsection{Writers are concerned about the devaluation of their work as a result of co-writing with AI}
Throughout the study, writers expressed concerns about audiences' reaction to them applying AI assistance for their writing.
While some believed readers might have split opinions depending on their level of acceptance of new technology, particularly AI, all of the writers expected to receive some negative feedback from readers.
Notably, in writers' view, ``readers'' include not only general audiences who might read and purchase their work but also the clients who directly determine the commissions of their writing jobs.
They were worried that their use of AI writing assistance---and the fact that anyone can use AI for text production---would result in lower perceived value and misperception of their writing as ``easy work'' (P13). 
Writers expressed increased concerns as adopting AI writing assistance has become more commonplace across various industries.
In the long run, they believed professional writers would continue to appreciate work from their peers, but they were uncertain whether non-experts, including some of their clients, would undermine the value of human writing as AI assistance becomes widely accessible. 
% \placeholder{mention something about the writer economy + authenticity as value for pay}


\subsubsection{Readers appreciated writers' attempt to explore new technology and expressed interest in reading AI-co-created text}
By contrast, readers in our study held a more positive view toward the use of AI writing assistance. Before actually reading these AI-co-written passages, readers' levels of interest are already significantly skewed toward the positive end ($\chi^{2} = 16.50$, $p < 0.001$).
The majority of them also believed work co-written with AI should be viewed as authentic writing as well ($\chi^{2} = 62.12$, $p < 0.001$). Readers also suggested whether a piece of work was co-written with AI would not affect how they evaluated and appreciated the writing ($\chi^{2} = 8.29$, $p < 0.081$).

\begin{figure}[h!]
    \centering
    \includegraphics[height=0.25\textwidth]{fig/part2_pre_rating.png}
    \caption{Readers' perceptions toward human-AI co-writing \textit{before} reading AI-assisted writing. Dashed lines represent mean values.}
    \label{fig:part2_psot_perception}
\end{figure}


After being disclosed that some of the passages they read were co-written with AI, readers expressed significantly more positive perceptions toward the writing ($\chi^{2} = 20.82$, $p < 0.001$) as well as the writer ($\chi^{2} = 55.94$, $p < 0.001$). This is a surprising result given that previous AIMC work often found readers to hold negative opinions towards the message and the writer once they are aware of the AI assistance~\cite{liu2022will,jakesch2019ai}. The qualitative responses reveals that, different from interpersonal communication with instrumental or relational purposes, leisurely readers focus on the writing outcome and their reading experiences, and are positive towards writers experimenting with new technology to improve the outcome. As one reader wrote in their open-text response: ``It [Using AI writing assistance] could indicate that the human writer is proactive in seeking innovative tools to enhance their creativity and productivity.''


\begin{figure}[h!]
    \centering
    \includegraphics[height=0.25\textwidth]{fig/part2_post_perception.png}
    \caption{Readers' perceptions toward the writing, the writer, and their approaches to evaluating work \textit{after} reading AI-assisted writing. Dashed lines represent mean values.}
    \label{fig:part2_psot_perception}
\end{figure}


Meanwhile, we also observed opinions toward perceived authorship become increasingly diverse. In particular, there is no significant trend in terms of whether humans or AI should receive more credits for AI-assisted writing ($\beta = 0.18$, $S.E. = 0.19$, $t = 0.97$, $p = 0.339$).
After all, they acknowledged applying AI tools to write has become more and more prevalent and agreed that the general public will eventually be more accepting of this practice.




%\subsection{Future of writing: Writers' desired AI assistance for authentic writing}
\subsection{The Help in Need: Building Personalized Feedback Loops}
\label{sec:future_support}

Likewise, writers also believed it is a matter of time for the public to accept and embrace co-writing with AI.
As such, many of them saw the benefits of exploring the tools and intended to start doing so with writing that ``requires less authenticity'' (P3).
These types of writing were described as grounded more in factual information (e.g., science writing, blog posts for product placement) and less on writers' personal experience and emotional expression.
As a general principle, writers hope future writing assistance tools could help them preserve their authentic voices in writing, but they prefer support that does \textit{not} come in the form of text production.
Instead, writers desire more support \textit{before} and \textit{after} the actual writing process and specifically pointed to two areas: (1) constructing fundamental materials for writing and (2) actively monitoring, analyzing, and providing feedback on writers' work.

In particular, writers hope to get help from AI to build \textbf{\textit{personalized feedback loops of good writing}}.
When asked how they would like to select writing samples to personalize their AI writing assistance, writers strongly preferred using their own popular work  (only 2 out of 19 writers would include work from others).
They also hoped AI could actively monitor and evaluate their writing, and most importantly, provide feedback on whether broader audiences would react positively to their work.
Specifically, they believed it would be the most helpful if AI could provide suggestions through an ``algorithmic point of view'' (P13), such as suggesting words that would be good for SEO optimization. 
But instead of directly receiving and adopting suggestions from the tool, writers would like to learn from such suggestions and incorporate them into their own writing.
% \placeholder{Mention something about writers' ideal of "good writing"}


\section{Discussion}

% Summary of the present work
In this work, we examined writer-centered conceptualizations of authenticity in human-AI co-writing.
We explored writers' desired approaches to preserving their authentic voices in writing, and we particularly investigated the effectiveness of personalization in serving this design goal.
Through semi-structured interviews with 19 professional writers and an online survey study of avid readers' perspectives, we found writers' conceptions of authenticity focus more on their internal experiences---particularly, how they shape and express their authentic self even before and throughout the writing process.
It is also through their situated practices of co-writing with AI that writers shape and re-shape their perceptions of authenticity in the context of human-AI co-creation.
Insights from our study not only provide critical design implications for future AI writing assistance but also practical guides---with an eye on writers' identities and ethics---for human-AI co-creation in general. % something about ethical concerns


\subsection{Extending and Crystallizing Conceptions of Authenticity in Human-AI Co-Writing}
We begin with consolidating the writer-centered definition of authenticity as the foundation for designing better AI writing assistance tools.
%Per our writer participants, the two aspects of authenticity does map to existing themes discussed in existing literature. 
Writers' references to the source of work (source authenticity) and writing outcomes (content authenticity) are related to the \textit{Source} and \textit{Category} themes of authenticity in existing literature, respectively~\cite{Auth_Humanity_Guignon_2008, Auth_Humanity_AMA_Lehman_2019, Auth_Humanity_Handler_1986}, although the emphasis on content authenticity was much less prevalent than what prior work would suggest.
In contrast, the writers in our study also centered the concept of authenticity around writers' internal experiences before and throughout the writing process.
Specifically, they highlighted the importance of absorbing, digesting, and internalizing information, knowledge, and their lived experiences to nourish their authentic selves and express them in writing.
Ultimately, this becomes their signature, uniquely justifying why a piece of work would not turn into its very shape if done by anyone else.
Based on these fundamental concepts, we next discuss how the design of human-AI co-writing tools can support writers' authentic selves, source authenticity, and content authenticity.


\subsection{Designing \textit{for Authenticity} Human-AI Co-Creation Tools through Personalization}
% The current form of personalization is helpful for creating positive writing experience (which might aid authenticity through their writing processes), but might not directly add benefits to preserving writers' authentic voices
% Instead, AI can provide more support through offering unique "machine point of view" + other forms of personalization
% For writers, authenticity in writing means much more than "sounding like themselves"
% In fact, writers know how to write with and sound like their own authentic writing. Instead, they need other form of support to preserve authenticity

Our findings highlight the importance of tool design as writers' perception of authenticity as well as whether they can justify authenticity in their writing is rooted in the \textit{practices} of co-writing with AI.
%Examining the effectiveness of personalization in preserving writers' authentic voices during their writing processes, 
%we found the current form of personalization (i.e., simulating writers' styles and personalizing through writing output) helps create positive writing experiences.
%in our study, we found that personalizing by e.g., trying to simulate writers' styles helps create positive writing experiences.
We compared how writers worked with personalized versus non-personalized AI writing assistance and found limitations in the current form of personalization (i.e., simulating writers' styles and tones through in-context learning with LLM).
While this might indirectly contribute to building writing experiences that allow writers to find joy and meaning in their writing jobs, the approach demonstrated benefits to directly preserve writers' authenticity for two reasons.
For writers, authenticity means much more than producing text that seems stylistically similar to their work.
And after all, writers themselves know the best how to compose writing that represents their own unique features; hence, AI providing support in this way yields marginal benefits.
Instead, writers seek AI's support beyond text production.
Specifically, participants' responses provide suggestions for how alternative forms of personalization could be more advantageous, which we further elaborate on below.

%\subsubsection{\textbf{Absorption comes before production: Supporting \underline{authentic self} through personalizing ``brain food''}} 
\subsubsection{\textbf{Internalization comes before text production: Supporting \underline{authentic self} through personalizing sources of writing inspiration}} 
% (1) to support the "internal states" aspect of authenticity
%%% (1.a.) AI as internalization tool to help nurish the "real materials" of writing
%%% (1.b.) AI keeping the writing flow
%%% (1.c.) personalization through providing materials for internalization
Our study suggests that authenticity could be supported by enriching the materials that writers digest and later on apply to (improve) their writing.
In the interviews, writers highlighted that the most important practice of ``writing'' is, in fact, to nurture themselves with rich information and experiences.
Many writers emphasized how reading plays an important role in improving their writing and how AI can efficiently support the process of synthesizing and internalizing large amounts of information. 
In this regard, personalizing materials for internalization can support authenticity by helping writers to enrich their authentic, intellectual selves---which are \textit{the} bases for authentic writing.


\subsubsection{\textbf{Going beyond the audience's flow: Supporting \underline{source authenticity} through personalizing writers' targets for growth}}
% (2) to support the "source" aspect of authenticity
%%% (2.a.) Our study highlights a lot of writers' concerns come from their insecurity toward readers' reaction --> AI to provide more hints of feedback from audiences. this might also support AI to support writers' expressing themselves more freely and genuinely 
%%% --> circle back to AI ghostwriting effect
%%% (2.b.) personalization through personalizing feedback
Across all conversations with writers, we saw how their uncertainty---and oftentimes insecurity---about audiences' responses set constraints to how freely they can express themselves in writing. 
Their concerns also explain why they are hesitant to declare AI's contribution to writing and resonate with the AI Ghostwriter Effect~\cite{HAIC_authenticity_AI_Ghostwriter_Effect}.
However, our survey in Part~2 suggests writers' worries might not necessarily align with readers' attitudes in reality.
To more directly tackle the ``source'' aspect of authenticity, we first recognize the need to communicate readers' feedback to writers.
Indeed, writers have already envisioned AI as a helpful tool to synthesize public opinions and preferences.
Here, we see opportunities for personalization such that writers could get feedback that is tailored to their interests and needs to shape their writing.
Furthermore, the feedback mechanisms should place more emphasis on helping writers decide what they want to achieve through their writing. 
In particular, offering support during the early stage of idea development (i.e., the ``fuzzy area'' that writers referred to) might be more effective in helping writers preserve their authenticity in writing. 
During this planning stage, they could more proactively decide what goes into the writing, serving their ``content gatekeeping'' job to make major contributions to writing.
Besides, referencing public interests for goal-setting---instead of following audiences' tastes to craft the actual writing pieces---can also help writers maintain their autonomy during the writing process.


\subsubsection{\textbf{Learning, not receiving: Supporting \underline{content authenticity} through personalizing active feedback}}
% (3) to support the "writing outcomes" aspect of authenticity
%%% (3.a.) Instead of directly getting content from AI, writers' want to *learn* from AI through feedback loops of good writing
%%% (3.b.) personalization through analysis, metrics, and other machine POV
As mentioned in the idea of building a ``feedback loop of good writing,'' writers are less interested in attaining good writing content from AI.
Instead, they are more motivated to learn how to improve and produce good writing through AI's feedback.
From our interviews, we also learned that what each writer targets and considers ``good writing'' varies widely from writer to writer.
Therefore, providing customized aids to help writers learn to improve their own writing in the ways they want to could be another promising use of personalization.
In our study, writers specifically sought ``machine points of view'' for active monitoring and in-text feedback from AI to improve their writing.
In this regard, enabling users to select and customize the types of metrics to use for analyzing their writing output can be a plausible starting point.


% \placeholder{Mention something about design of for-authenticity tools need to take a more holistic approach; to support the growth of writers from the ground-up, not just the quality of content per se. Because as writers grow, their writing flourishes as well.}
%All in all, the design of for-authenticity AI co-creation tools should take a more holistic approach, 
All in all, designing AI co-creation tools that preserve authenticity should take a more holistic approach, 
such that AI assistance is \textit{not} narrowly focused on the writing process and output per se. 
Instead, the designers and developers of these tools should \textbf{\textit{target the growth of writers as their ultimate design goal}}.
This can be done through enriching materials that writers consume and by helping writers learn through public feedback and analyses of one's work.
As writers grow, they might seek different topics, content, and styles in their writing. 
Therefore, personalizing their ways of writing might offer only temporary aids but risk depriving their sense of ownership and control in writing~\cite{HAIC_authenticity_choice_over_control}.
As writers grow, they need support not only for improving the quality of their work but also for them to thrive intellectually. %and mentally.
Therefore, it is critical to diversify sources of inspiration and build more healthy relationships with feedback from the wider crowds.
And most importantly, as writers grow, their writing flourishes as well.


\subsection{Writer-Reader Relationship in the Age of Human-AI Co-Creation}
% inconsistent view between writers and readers
Contrasting the findings from Part~1 and Part~2 of our study, we found apparent differences between writers' versus readers' views.
Unlike writers' concerns, readers could not tell when writers applied AI assistance but reacted more positively to the idea of experimenting with AI co-writing.
This highlights a fundamental difference between how writers and readers judge the \textit{value} writing output.
For writers, valuation is rooted in the hard work that goes into conceiving and producing content; for readers, valuation is based on the outcomes of work per se, and they
%While writers are concerned about readers' responses to human-AI co-creation, it is important to note that audiences 
do not appear to associate AI-assisted work with either loafing or effortlessness.
In fact, recent work has suggested working with AI assistance could even demand more work from creators~\cite{AIwriting_Tool_integrative_leap_multimodal}.
The connection between writers and readers remains bonded through the output of writing pieces.
Therefore, devaluation of work will more likely arise when writers fail to deliver quality work that meets readers' expectations---which do not entail promises for \textit{how} the work is made.


\subsection{What AI Writing Assistance is (Not): Generalizability and Boundaries of the Present Insights}
% compare and contrast AIMC vs. AI writing assistance

Providing more clarity to how authenticity is conceptualized in human-AI co-writing also clarifies the distinction between AI-assisted writing and other relevant realms, particularly AI-mediated communication (AIMC).
By comparing and contrasting the two topics, we further address generalizability of the present research.
AIMC adopts AI assistance to produce content for \textit{two-way} communication~\cite{AIMC_Hancock_JCMC_2020}.
This entails delivering messages and meanings to and expecting reciprocal interaction from target recipients.
Here, the term ``mediation'' captures the nature of the type of context where the writing happens adequately, implying a more participatory role of AI as it possibly alters dialogues between communicators.
On the other hand, while co-writing with AI in more creative settings also produces content, this content is often delivered one-way to a larger crowd and does not involve a bi-directional message exchange between writers and readers.
Furthermore, our study reveals the practice of writing spans far beyond crafting the content per se, and conveying messages to the audience is simply the final step.
Given these distinctions, we expect insights of the present work more appropriately apply to comprehend AI's role in facilitating (1) unilateral presentation of content to a group of individuals and (2) creative practices that nurture the creators and enrich their work; while these practices can span beyond the content production phase.


\subsection{Limitation and Future Work}
Despite our best efforts and mixed-methods approach to studying this topic, we acknowledge several limitations of the present work as well as the fast-changing landscape and public sentiment in the AI space.
To begin with, data collection of the present work took place from June to October of 2023. 
This is a unique timing as the public has somewhat been exposed to the popular trend of generative AI and its use for text production, but has not yet moved to complete acceptance and adoption of the new technology.
During this period, new applications of AI writing assistance are also being deployed day in and day out.
Therefore, we also expect writers, readers, and the general public's opinions toward this topic to shift over time.

Moreover, as abundant media coins the term ``AI hype'' throughout the year of 2023, we suspect responses from both our writers and readers might more or less be affected by popular discussions about generative AI.
We encourage future work to examine trends across time, capturing and following how writers' and readers' responses change through longitudinal research.
In particular, an interesting topic to explore is whether any of these attitudinal or behavioral changes occur due to advances in new AI applications or due to changes in public regulations, media depictions, or other external factors.

As both our writer and reader participants carry along unique characteristics, on one hand, these contextual factors add value and richness to the present work.
On the other hand, future work should consider conducting larger-scale studies, surveying both experts and non-experts as well as dedicated and regular audiences. 
This allows one to better account for the influences of participants' positionalities on their views toward authenticity. Moreover, our study only examined a limited scope of readers and writer-reader relationship. Specifically, the readers were passively and leisurely consuming the wiring we provided, where their focus on the ``reading experience'' over the writer was more heightened. Our results may not generalize to readers who actively seek out work from a particular author, or take personal interest in the writer. 

Finally, though we supplement writers' perspectives with readers', our focus remains on writing as creative work and has not captured views from other stakeholders (e.g., writers' clients) who contribute to the profitable drive of this industry.
We have not yet thoroughly explored how the changing writer economy might affect writers' decisions and work, while participants have also hinted at possible influences.
Therefore, we encourage future work to further explore the impact of human-AI co-creation on the monetization of creative work.


% \section{Conclusion}


% Vera's comments

% -the different asepcts of authenticity are really interesting. How to support each? Are there less obvious opportunities for AI-wiriting tools? Are there tensions?

% -what is the relation between authenticity and other constructs studied in previous work, such as ownership, control, agency (maybe worth taking a look at Hannah’s dissertation: https://www.proquest.com/openview/663ef172abb7a18bfee145301e322f63/1?pq-origsite=gscholar&cbl=18750&diss=y)? I am also curious if the results can help explain the “AI ghostwriter” effect, that authors do not perceive ownership, but still assign authorship (categorically mine? Internal state?)

% -dig deeper on personalization: does in-context learning help satisfy some aspects of authenticity but not others? Is the current approach not enough or miss some opportunities for authenticity? Can we give authors other personlization/control mechanisms that help?

% -writer-reader inconsistency: why readers do not perceive difference between personalized v.s. Non-personalized (acknowledge possible study limitations: e.g. not enough exposure to original styles), and perceive AI-supported writing positively? Some possible hypothesis: subject population biased towards AI positivity; assign authenticity to author+AI; care more about content instead of author in leisurely reading (authenticity is less of a value for readers of leisurely reading?)

% -relatedly to above, how our results extend AI mediated communication literature? E.g., Types of communication matter; attribution to what (content v.s. communicator); 

% - we have to be careful not to oversell the point that “readers do not care/like it better”. One is to acknowledge the possible bias of population/timing of public perception with genAI; the other is to discuss other (long-term) negative effects on writers and reader-writer relationship


==> archived/results_old_version.tex <==
\subsection{Defining authenticity in creative writing with AI [RQ1]}
% Results from qual interviews
Authenticity represents the identity of a writer behind a story. These identity markers are rooted in writers' cultural backgrounds, individual experiences, situated environments, and more. They can be manifested through various forms in writing, such as writers' unique tones, uses of language, original ideas, and emotional appeals. Whether an author can genuinely express their identity through these above-mentioned forms shapes the authenticity of writing.

\begin{itemize}
    \item Authentic writing is about the story that's told from the heart of an author. If there is no human behind the story, it wouldn't be as meaningful. And writing would just be pieces of words.
    \item A large part of authenticity comes from the experience and environment that the creators are situated in.
    \item Everyone starts with similar ideas but individual experiences allow for personal, unique ways of storytelling.
\end{itemize}


After trying out the AI writing tools, all writers agreed that co-writing with AI \textit{is} authentic writing since human writers still did most of the work.
Here, the amount of work centers on the degree to which one makes active decisions during the writing process.
As writers prompted and received generative output from AI, they went through this negotiation process of whether to accept or reject/revise content from the tools.
If one takes control and makes deliberate decisions over the direction of content, instead of passively accepting, copying, and pasting output from AI, then co-writing with AI remains a form of authentic writing.

Another argument for why co-writing with AI is authenticity has to do with \textit{internalization} as a core practice of writers.
Writers constantly read, synthesize, and learn from others' writing to improve their own as a part of their day-to-day job.
There is a fine line between such practice and plagiarism as what writers typically do is to absorb what they like from others' work and then internalize, transform, and adapt them to their own approaches to writing.
They consider such an exercise very similar to what AI does, but it is able to process and compress such work within an extremely short amount of time.
In other words, if co-writing with AI is \textit{not} authentic writing, then perhaps authentic writing does not at all exist.



\subsection{Impact of AI on creative writing [RQ2, RQ3]}

% Results from qualitative interviews
\subsubsection{Impact on authenticity in writing}
Based on writers' comments in the qualitative interviews, whether AI affects authenticity in writing again depends on whether writers actively step in to make deliberate decisions in writing. 
The use of AI per se does not undermine authenticity in writing.

\subsubsection{Impact on writing processes and outcomes}
% Impact on efficiency/productivity
Writers hold split opinions about AI's impact on the efficiency and productivity of writing.
On one hand, AI allows for speedy content generation; on the other hand, having to go back and forth editing AI generative output might take more time compared to writers' normal work.
Writers do acknowledge that AI is of great help in extending the length of content, which is often how professional writers are paid (e.g., payment by word count).


% Impact on creativity
Writers do recognize AI's benefits in offering ``jumping points'' to remove writing blocks. This not only helps create a smoother flow in writing but also serves the potential to enhance creativity.
As various writers mentioned they use the AI tool as inspiration, looking at the variety of AI generative output (in terms of ideas and formats) can often lead writers to directions that they might not pursue by themselves. 


% Impact on synthesizing audience's values
Writers see LLM output to serve as representations of the general public and syntheses of online information.
In this regard, they expect AI can have positive influences on their writing such that they can better take into account the preferences and interests of general audiences.


% Results from behavioral data via writing log
We contrast writers' qualitative feedback with their behavioral data by analyzing their writing logs...


\subsection{Writer-centered needs and considerations for AI writing assistance [RQ4, RQ5]}

\begin{itemize}
    \item AI as a prototyping tool to plan for writing
    \item AI as a Q\&A tool to synthesize materials for writing
    \item AI as an optimization tool for popularity
\end{itemize}

% AI as a prototyping tool to plan for writing
AI can be a great tool to help writers see how things will look like if they structure their writing in different ways. 
\begin{quote}
    It's almost like you put all the text you have into, like I said before, a kind of synthesizer, and then they would give you, okay, here are three different plans. Plan A, B, and C, and you can compare and contrast. -- P10
\end{quote}


% AI as a Q\&A tool to synthesize materials for writing
Writers need to ask themselves a lot of questions during the writing process, and AI can be a great tool for Q\&A.
\begin{quote}
    I tend to ask a lot of questions because I think that's a way to keep the reader's attention. But I'm not going to ask only questions because then it doesn't really make any sense to the reader. So I need to ask a question, then I need to try to answer it in some way. And I think that AI is probably very good at that, providing five possible answers to a question.  -- P12
\end{quote}


% AI as an optimization tool for popularity
AI can help with providing guides that optimize for search and SEO, such as hinting at optimal word choices that yield better SEO outcomes, which is also what writers are rewarded for in their professional work.
\begin{quote}
    If I am working on a novel or a poem, I don't know if AI would give me something that fits my tone, something that's unique, something that it's not my idea, and I wouldn't feel comfortable using it if it wasn't my idea. Versus if I'm using it for SEO writing, I could see it being really helpful to kind of go through some of the text and be like, oh, you need to optimize some of these keywords. I can see a lot of opportunities that ... it's more by the book. That's more objective. -- P03
\end{quote}



\subsection{Personalization of AI writing assistance [RQ6]}
Writers prefer working with an AI that doesn't sound exactly like themselves but still produces similar styles so that they can easily adapt AI output to their own writing through light editing.
In this regard, writers often prefer working with the AI tool with in-context learning. This does not guarantee that AI-generated output sounds more similar to the writers' unique voices, but oftentimes, they could more readily revise and adapt AI suggestions to their own writing.

==> table/table_reader_genre.tex <==

\begin{table}[h!]
    \centering
    \begin{tabular}{p{0.35\textwidth}|p{0.35\textwidth}}
    \toprule
        \textcolor{blue}{Genre} & \textcolor{blue}{Percentage of reader participants who frequently read the genre}  \\ 
        \hline
        \textcolor{blue}{Fantasy} & \textcolor{blue}{67.03\%} \\
        \hline
        \textcolor{blue}{Science fiction} & \textcolor{blue}{66.49\%} \\
        \hline
        \textcolor{blue}{Romance} & \textcolor{blue}{64.32\%} \\
        \hline
        \textcolor{blue}{Contemporary fiction} & \textcolor{blue}{63.24\%} \\
        \hline
        \textcolor{blue}{Thrillers and horror} & \textcolor{blue}{62.70\%} \\
        \hline
        \textcolor{blue}{Mystery} & \textcolor{blue}{22.16\%} \\
        \hline
        \textcolor{blue}{Historical fiction} & \textcolor{blue}{20.00\%} \\
        \hline
        \textcolor{blue}{Inspiration and self-help} & \textcolor{blue}{17.84\%} \\
        \hline
        \textcolor{blue}{Biography, autobiography, and memoir} & \textcolor{blue}{6.49\%} \\
        \hline
        \textcolor{blue}{Poetry} & \textcolor{blue}{2.16\%} \\
        \hline
        \textcolor{blue}{Drama and screenplay} & \textcolor{blue}{1.62\%} \\
        \bottomrule
    \end{tabular}
    %\caption{Frequently read literature genres by reader participants in Part~2}
    \label{tab:reader_genre}
\end{table}
